Towards Faster Decentralized Stochastic Optimization with Communication Compression

Communication efficiency has garnered significant attention as it is considered the main bottleneck for large-scale decentralized Machine Learning applications in distributed and federated settings. In this regime, clients are restricted to transmitting small amounts of quantized information to their neighbors over a communication graph. Numerous endeavors have been made to address this challenging problem by developing algorithms with compressed communication for decentralized non-convex optimization problems. Despite considerable efforts, the current results suffer from various issues such as non-scalability with the number of clients, requirements for large batches, or bounded gradient assumption. In this paper, we introduce MoTEF, a novel approach that integrates communication compression with Momentum Tracking and Error Feedback. Our analysis demonstrates that MoTEF achieves most of the desired properties, and significantly outperforms existing methods under arbitrary data heterogeneity. We provide numerical experiments to validate our theoretical findings and confirm the practical superiority of MoTEF.

==> macros.tex <==
\RequirePackage{xcolor}
\usepackage{amsmath,amsthm}
\usepackage{comment}
\usepackage{multirow}
%\usepackage{cite}
\usepackage[numbers]{natbib}
\usepackage{graphicx}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{threeparttable}
\usepackage{makecell}
\usepackage{pifont} 
\newcommand{\makecellnew}[1]{{\renewcommand{\arraystretch}{0.8}\begin{tabular}{c} #1 \end{tabular}}}


\usepackage[english]{babel}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{nicefrac}
\usepackage{lmodern}
%\usepackage[flushleft]{threeparttable}
\usepackage{epigraph}
\usepackage{subcaption}
\usepackage{csquotes}
\usepackage{booktabs}
\usepackage{geometry}
\geometry{left=2.5cm}
\geometry{right=2cm}
\geometry{top=2cm}
\geometry{bottom=2cm}


\usepackage{thm-restate}
\usepackage{empheq}
\usepackage{ bbold }
\usepackage{authblk}
\usepackage{color}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\newcommand{\purple}{\color{purple}}
\newcommand{\teal}{\color{teal}}
\newcommand{\algname}[1]{{\small \sf#1}}
\usepackage[pagebackref]{hyperref}

\hypersetup{
	colorlinks=true,        % false: boxed links; true: colored links
	linkcolor=blue,         % color of internal links
	filecolor=magenta,
	citecolor=darkgreen,         % color of links to bibliography
	urlcolor=blue           % color of external links
}
\renewcommand*{\backrefalt}[4]{%
    \ifcase #1 \footnotesize{(Not cited.)}%
    \or        \footnotesize{(Cited on page~#2)}%
    \else      \footnotesize{(Cited on pages~#2)}%
    \fi}
\usepackage{cleveref}
% \usepackage{cite}
%\usepackage{framed}
\usepackage{tikz-cd} 
\usepackage{algorithm}
\usepackage{algpseudocode}
\usetikzlibrary {graphs} 
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{arrows.meta}

\tikzstyle{node} = [rectangle, rounded corners, 
minimum width=1cm, 
minimum height=0.5cm,
text centered, 
draw=black, 
fill=white]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{doublearrow} = [thick,<->,>=stealth]

\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,47,25}
\definecolor{mydarkblue}{RGB}{39,47,180}


%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% THEOREMS 
%%%%%%%%%%%%%%%%%%%%%%%%%

%change numbering if needed

\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem{definition}{Definition}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{example}[lemma]{Example}

%\newtheorem{remark}{Remark}
%\newtheorem{corollary}{Corollary}
%\newtheorem{example}{Example}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}%

\newcommand{\prev}{\text{prev}(k,i_k)}
\newcommand{\avg}{\text{avg}}
\newcommand{\Prev}{\text{prev}}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Ek}[1]{\mathbb{E}_k\left[#1\right]}
\newcommand{\EE}{\mathbb{E}}

\newcommand{\abccond}{$\alpha$-$\beta$-condition }
\newcommand{\ft}{\widetilde{f}}
\newcommand{\xt}{\widetilde{x}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cX}{\mathcal X}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\mSigma}{\mathbf{\Sigma}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\wtilde}[1]{\widetilde{#1}}
\newcommand{\wtau}{\widetilde{\tau}}

\newcommand{\proj}{{\rm Proj}}


\providecommand{\Eb}[1]{{\mathbb E}\left[#1\right] }       %expectation, with brackets
  \providecommand{\EE}[2]{{\mathbb E}_{#1}\left.#2\right. }  %expectation  
  \providecommand{\EEb}[2]{{\mathbb E}_{#1}\left[#2\right] } %expectation,  with brackets
  
\renewcommand{\empty}{\varnothing}
%\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{\coloneqq}
\newcommand{\avein}{\frac{1}{n}\sum_{i=1}^n}
\newcommand{\sumin}{\sum_{i=1}^n}
\newcommand{\lrin}{\gamma_{w}}
\newcommand{\lrout}{\gamma_{\theta}}
\newcommand{\lroutm}{\gamma_{\theta,m}}



\newcommand{\lr}[1]{\langle #1\rangle}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\Next}{next}
%\DeclareMathOperator{\Prev}{prev}
\def\<#1,#2>{\langle #1,#2\rangle}
\newcommand{\squeeze}{\textstyle}




\newcommand{\cC}{\mathcal{C}}
%\newcommand{\cR}{\mathcal{R}}
%\newcommand{\cS}{\mathcal{S}}
%\newcommand{\cD}{\mathcal{D}}
%\newcommand{\cI}{\mathcal{I}}
%\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal M}
%\newcommand{\cN}{\mathcal N}
\newcommand{\cQ}{\mathcal Q}
\newcommand{\diff}{\mathrm{d}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\clip}{clip}

\usepackage[colorinlistoftodos,bordercolor=purple,backgroundcolor=pink!20,linecolor=pink,textsize=scriptsize]{todonotes}
\newcommand{\TODO}[1]{\todo[inline,linecolor=green,backgroundcolor=green!25,bordercolor=green,caption={}]{#1}}
\newcommand{\aurelien}[1]{\todo[inline,caption={}]{\textbf{Aurelien: }#1}}
\newcommand{\rustem}[1]{\todo[inline,caption={}]{\textbf{Rustem: }#1}}
\newcommand{\eduard}[1]{\todo[inline,caption={}]{\textbf{Eduard: }#1}}
\newcommand{\samuel}[1]{\todo[inline,caption={}]{\textbf{Samuel: }#1}}


\def\toptitlebar{\hrule height1pt \vskip .25in} 
\def\bottomtitlebar{\vskip .22in \hrule height1pt \vskip .3in} 

\newcommand{\circledOne}{\text{\ding{172}}}
\newcommand{\circledTwo}{\text{\ding{173}}}
\newcommand{\circledThree}{\text{\ding{174}}}
\newcommand{\circledFour}{\text{\ding{175}}}
\newcommand{\circledFive}{\text{\ding{176}}}
\newcommand{\circledSix}{\text{\ding{177}}}
\newcommand{\circledSeven}{\text{\ding{178}}}
\newcommand{\circledEight}{\text{\ding{179}}}
\newcommand{\circledNine}{\text{\ding{180}}}
\newcommand{\circledTen}{\text{\ding{181}}}
\newcommand{\circledEleven}{\text{\ding{182}}}
\newcommand{\circledTwelve}{\text{\ding{183}}}


\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{darkred}{\ding{55}}}%




\definecolor{BrickRed}{RGB}{143,20,2}
\definecolor{PineGreen}{RGB}{0,110,51}

\newcommand{\revision}[1]{{\color{BrickRed}#1}}
\providecommand{\0}{\mathbf{0}}
  \providecommand{\1}{\mathbf{1}}
  \renewcommand{\aa}{\mathbf{a}}
  \providecommand{\bb}{\mathbf{b}}
  \providecommand{\cc}{\mathbf{c}}
  \providecommand{\dd}{\mathbf{d}}
  \providecommand{\ee}{\mathbf{e}}
  \providecommand{\ff}{\mathbf{f}}
  \let\ggg\gg
  \renewcommand{\gg}{\mathbf{g}}
  \providecommand{\hh}{\mathbf{h}}
  \providecommand{\ii}{\mathbf{i}}
  \providecommand{\jj}{\mathbf{j}}
  \providecommand{\kk}{\mathbf{k}}
\renewcommand{\ll}{\mathbf{l}}
  \providecommand{\mm}{\mathbf{m}}
  \providecommand{\nn}{\mathbf{n}}
  \providecommand{\oo}{\mathbf{o}}
  \providecommand{\pp}{\mathbf{p}}
  \providecommand{\qq}{\mathbf{q}}
  \providecommand{\rr}{\mathbf{r}}
  \providecommand{\ss}{\mathbb{s}}
  \providecommand{\tt}{\mathbf{t}}
  \providecommand{\uu}{\mathbf{u}}
  \providecommand{\vv}{\mathbf{v}}
  \providecommand{\ww}{\mathbf{w}}
  \providecommand{\xx}{\mathbf{x}}
  \providecommand{\yy}{\mathbf{y}}
  \providecommand{\zz}{\mathbf{z}}

  \providecommand{\Eb}[1]{{\mathbb E}\left[#1\right] }  

  \definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{darkred}{rgb}{0.8,0.,0.0}


  \providecommand{\mG}{\mathbf{G}}
  \providecommand{\mH}{\mathbf{H}}
  \providecommand{\mI}{\mathbf{I}}
  \providecommand{\mJ}{\mathbf{J}}
  \providecommand{\mK}{\mathbf{K}}
  \providecommand{\mL}{\mathbf{L}}
  \providecommand{\mM}{\mathbf{M}}
  \providecommand{\mN}{\mathbf{N}}
  \providecommand{\mO}{\mathbf{O}}
  \providecommand{\mP}{\mathbf{P}}
  \providecommand{\mQ}{\mathbf{Q}}
  \providecommand{\mR}{\mathbf{R}}
  \providecommand{\mS}{\mathbf{S}}
  \providecommand{\mT}{\mathbf{T}}
  \providecommand{\mU}{\mathbf{U}}
  \providecommand{\mV}{\mathbf{V}}
  \providecommand{\mW}{\mathbf{W}}
  \providecommand{\mX}{\mathbf{X}}
  \providecommand{\mY}{\mathbf{Y}}
  \providecommand{\mZ}{\mathbf{Z}}

  \providecommand{\norm}[1]{\left\lVert#1\right\rVert}
\providecommand{\EEb}[2]{{\mathbb E}_{#1}\left[#2\right] } 

\providecommand{\EbNSq}[1]{\Eb{\norm{#1}^2}}
  \providecommand{\EbNFSq}[1]{\Eb{\norm{#1}_{\rm F}^2}}

  
